From Trust to Appropriate Reliance: Measurement Constructs in Human-AI Decision-Making

While human-AI decision-making research has primarily used trust measurements to assess the practical usage of AI systems by their end-users, recent empirical evidence suggests that trust measurements do not inform users' appropriate reliance on AI systems. While examining the human-AI decision-making literature, in this work, we review empirical studies that assess people's appropriate reliance on AI advice, differentiating measurements and constructs of appropriate reliance from trust and mere reliance. Our analysis of literature shows that constructs for human-AI appropriate reliance are still fragmented in research. We present three views on appropriate reliance, namely Traditional, Appropriateness, and Dominance, as discussed in research. Using these views, we evaluate objective metrics reported in studies and argue for their consensus to facilitate the comparison across empirical research. We also discuss how studies employ objective metrics and examine their validity in application contexts. Our work contributes to the critical body of research on exploring objective metrics for assessing humans' appropriate reliance on AI advice.

==> tables/extras.tex <==
AI systems are being increasingly deployed in various domains to assist human decisions. 
In human-AI decision-making, AI advice is used to enhance decisions while maintaining human autonomy.
However, a known phenomenon is that humans often do not appropriately rely on AI advice.
While recent research has started to understand how humans build reliance on AI advice, we argue that it largely overlooks an important aspect: failing to replicate human-realistic decision-making scenarios.
AI systems, Human factors, and interaction methods influence reliance in human-AI decision-making.
To better understand these aspects and their interplay, we conduct an analytical review of recent studies in human-AI reliance literature. 
We summarize how Human-Computer Interaction (HCI) researchers study human-AI reliance, differentiating from the existing notion of trust.
Our findings show that studies aim to engage users with AI advice to avoid inappropriate reliance; however, they often fail to extract realistic user behavior.
We assess the interventions used to study AI reliance and their validity in application-grounded contexts.
We also discuss the research progression towards \textit{``consensus on what factors contribute to appropriate reliance on AI-Advice.''}
While outlining this progression, we discuss research gaps and make recommendations for further research on intervention designs.
Overall, this article outlines the need to develop uniform frameworks for building appropriate reliance on AI advice.


Collectively, these dimensions are highly fragmented, and a critical evaluation is necessary to bridge the open gaps between studies. 

The focus on human behavior with AI-assisted has gained interest recently, with evidence from studies showing over-reliance on AI advice~\cite{schemmer2023appropriate, schemmer2023towards}.

Such behavior can also be attributed to users' cognitive biases~\cite{lu2021human} (e.g., automation bias), lack of system understanding~\cite{morrison2024impact, cao2024designing}, or self-efficacy~\cite{ma2024you, chiang2022exploring, he2023knowing} in decision-making.

Positive first impressions can lead to automation bias and more errors as the user is overconfident in not only the model’s strengths but also the weaknesses of the system, and they generally over-rely on the system~\cite{nourani2021anchoring}. 

Yin et al.~\cite{yin2019understanding} focus on the interpretation of performance metrics such as model accuracy. 

They ~\cite{schoefer2024explanations} explore deeper factors into AI reliance on fairness, exploring the effect was seen as gender, by predicting more women to be professors.

Findings raise doubts about the reliability of popular feature-based explanations as enablers for distributive fairness.

Cognitive forcing functions~\cite{buccinca2021trust} reduce overreliance, but affect usability and acceptability. 


Schemmer et al~\cite{schemmer2023appropriate} also clarify that reliance is not binary (achieved or not achieved), but a degree of AR can also be achieved.

Helping non-expert users understand uncertainty~\cite{yin2019understanding}.

The idea behind human-AI decision-making is to be more effective than both human and AI individually~\cite{dellermann2019hybrid}.
True potential lies in leveraging human capabilities. CTP is not achieved due to poor human performance~\cite{bansal2021does, schemmer2023appropriate}, but human-AI decision-making is the optimal way forward. 
He et al.~\cite{he2023stated} chose a loan prediction task to see the risk and benefit and study the effect of analogies on prediction accuracy. 

Feature-based approaches are less effective than example-based approaches~\cite{chen2023understanding}. 

In reality, decisions are made for the future, and people will not know whether their predictions are correct or wrong; however, understanding their behavior can help improve these decisions~\cite {grgichlaca2019human}.

The consequential decisions, e.g., jailing or bailing, affect people's tendency to delegate tasks to machines~\cite{grgichlaca2019human}.
ML decisions are probabilistic, as compared to deterministic, which means there is never a guaranteed correctness~\cite{zhang2020effect}. 


Highly complementary performance requires adapting beyond confidence~\cite{bansal2021does}.
Design based on the frequency of agreement between HAI~\cite{bansal2021does}. 


Brachman et al.~\cite{brachman2022reliance} study human-AI labeling tasks to improve the efficiency and accuracy of conflict resolution in a banking scenario.
In this work~\cite{brachman2022reliance}, they focus on users' decisions to use this automation and support users in making manual decisions for challenging conflicts. 

Including the domain knowledge of expert users should allow less expert users to make better decisions~\cite{dikmen2022effects}.

Single controlled experiment with a single task and with crowd-workers~\cite{buccinca2025contrastive}. 
Adapting AI performance to individual traits can be used to enhance reliance~\cite{swaroop2024accuracy}.
Issues with complex domains with lay users~\cite{swaroop2024accuracy}.



Chen et al.~\cite{chen2023understanding} use a different style where they gave all tasks without AI assistance, and then randomly showed the same tasks with AI assistance, which is somehow problematic, as it is more about remembering the tasks rather than concentrating on AI support for the same task. 

Explanations reduce over-reliance in difficult tasks~\cite{vasconcelos2023explanations}. 
Explanations that make the AI’s mistake obvious reduce over-reliance~\cite{vasconcelos2023explanations}.

Participants who overestimated their performance demonstrated an increased appropriate reliance~\cite{he2023knowing}.


Uses the judicial system where a decision has to be made in favor of or against someone~\cite{cabitza2025oracular}. The oracular (traditional) AI support and the judicial AI support~\cite{cabitza2025oracular}. Evaluate whether the judicial AI protocol negatively impacts diagnostic accuracy~\cite{cabitza2025oracular}.

Significant effect on humans’ level of expertise on the effect of explanations’ correctness~\cite{morrison2024impact}.
Visual, example-based explanations are more deceptive than natural language explanations~\cite{morrison2024impact}.
The language tone of explanations does not impact humans’ decision-making behavior~\cite{morrison2024impact}.

There is a need to support high-complexity and prognostic tasks in human-AI decision-making~\cite{salimzadeh2024dealing}.

The effect of language tone on humans’ appropriate reliance when interacting with imperfect XAI underexplored~\cite{morrison2024impact}.

Explore incorrect explanations, even when the AI’s advice is correct~\cite{morrison2024impact}.

Diagnostic tasks involve situations where participants are provided with detailed and comprehensive information about the task, (theoretically) enabling them to make accurate decisions.


AI systems can also be improved with correct representations of users' mental models~\cite{schemmer2023towards, prabhudesai2023understanding}.

For instance, automation bias and algorithmic aversion are key user traits that influence their behavior~\cite{pareek2024effect, he2023stated}.

Overestimation of performance will result in under-reliance, and Poor performance can be due to the illusion of superiority of AI systems~\cite{he2023knowing}.
Users overestimate their competence and performance, which affects user reliance on AI systems~\cite{he2023knowing}.
Schemmer et al.~\cite{schemmer2023towards} study the effect of learning (expertise) on AR and how explanations affect task-specific learning.
He et al.~\cite{he2023knowing} propose to leverage tutorials to calibrate their self-assessment by revealing the actual performance level of participants with performance feedback.
Contrastive explanation can also help, when users refrain from trusting the system~\cite{he2023knowing}. 
Results indicate that such an intervention is highly effective in calibrating self-assessment (significant improvement), and has some positive effect on mitigating under-reliance and promoting appropriate reliance (non-significant results)~\cite{he2023knowing}.

Research looks closely at the effects of self-assessment in human-AI collaboration~\cite{he2023knowing}.

Ma et al.~\cite{ma2024you} propose a human self-confidence calibration to improve reliance. 
The difficulty of tasks affects human performance~\cite{schemmer2023appropriate}. 

Other factors combine mental models~\cite{zhang2020effect}, personality traits~\cite{swaroop2025personalising}, explanation appearance (text, graph)~\cite{yang2020how}, and decision-maker's intuition~\cite{ma2024you}.

Outcome: This approach directly assesses appropriate reliance based on the correctness of AI recommendations and human decisions~\cite{ma2024you}.
Can measure confidence on the task level and instance level. Higher accuracy with higher confidence shows positive results~\cite{ma2024you}. 

Cao et al.~\cite{cao2024designing} explore how model uncertainty presentation to foster appropriate reliance. (no model uncertainty, raw probability-based, calibrated probability-based, calibrated frequency-based).
Significant benefit of showing the calibrated uncertainty~\cite{cao2024designing}.

Facilitate people’s understanding of their decision-making performance. (e.g., ask people to make decisions on historical data and provide performance feedback)~\cite{lu2021human}.
Development of ML-based decision aids should not be isolated from the people who will use them~\cite{lu2021human}.
An unanswered question in this context pertains to why users tend to under-rely on AI systems despite their relatively high stated accuracy~\cite{he2023stated}.
Hence, research should further explore the effects of providing feedback to users on their performance~\cite{he2023stated}.

There is a high need to enable people to understand their decision-making first~\cite{lu2021human}, building models to assess their decision-making on historical data to understand their biases. 

Cabrera et al.~\cite{cabrera2023improving} propose directly showing end-users insights into AI behavior. E.g., behavior descriptions, details of an AI’s performance (metrics, common patterns, potential failures, etc.). For example, this model is 40\% accurate most of the time on text with 50 or fewer words.

Showing a behavior description enhances reliance~\cite{cabrera2023improving}. 

Acknowledge generalization of the results is the tasks selected for the experiments~\cite{cau2023effects}.

Users rely more on the instance data in case of a low-confidence prediction~\cite{cau2023supporting}.
A significant positive effect of the abductive and deductive explanation styles on task performance occurs when the AI confidence is high~\cite{cau2023supporting}.
When the AI confidence is low, our results suggest that it would be better not to explain the AI’s prediction~\cite{cau2023supporting}.

Peng et al.~\cite{peng2024human} Study user proficiency, AI agent capability, and their interaction effects on influencing the responses of users in IDSS.
Also enhances the effect of how the embodied AI affects user reliance on AI assistance~\cite{peng2024human}. 

Calibrated model confidence did not change users' perception~\cite{cao2024designing}. 

This may be because all the participants in this study were novices in the task. Limited size and unrelated to tasks (to novices) may not generalize to other domains that involve domain experts~\cite{cao2024designing}.


Benefits were only observed in showing the calibrated frequency presentation~\cite{cao2024designing}.
Design opportunity for personalized and adaptive human-AI collaboration~\cite{cao2024designing}.
Explanations improve decision-making when human and AI systems have comparable performance, and correcting each other is optimal~\cite{bansal2021does}. ut does not guarantee team complementarity. 


First, use a logical reasoning task to check people's self-assessment~\cite{he2023knowing}.

People with an AI background to test a domain-specific application for domain users, and pointed out that people are engaged~\cite{chen2023understanding}. 

Example-based explanations are drawn from training data and may not depend on the model. 

Cabitza et al.~\cite{cabitza2023ai} explore the theory of technology dominance~\cite{sutton2022extension}, and use the reliance and dominance as constructs to evaluate user reliance on AI-assisted decision making. 

Local explanation increases user performance, i.e., decision accuracy, and decreases task load more than other types of explanation~\cite{vered2023effects}.


AI correctness does not change the user’s performance~\cite{cau2023supporting}.
Acknowledging that we tried to replicate a realistic stock trading scenario, we also tried to minimize the interface burden for users with no experience in stock trading~\cite{cau2023supporting}.
Humans generate their explanations and benefit from them in the context of visual decision-making tasks~\cite{morrison2023evaluating}


The sample was biased toward more highly educated and ML-experienced individuals than the general population~\cite{chen2023understanding}.
Prabhudesai et al.~\cite{prabhudesai2023understanding} study the effect of communicating uncertainty on user reliance.

Uncertainty quantification, uncertainty communication, and transparent model reporting mechanisms are important factors for users~\cite{prabhudesai2023understanding}.


How the unique characteristics of uncertainty in ML models affect Human-AI interaction~\cite{prabhudesai2023understanding}. Linking existing tools helps shape understanding~\cite{prabhudesai2023understanding}. 
Match decisions with values~\cite{prabhudesai2023understanding}.
Match with mental models~\cite{prabhudesai2023understanding}.
Competence of the algorithm~\cite{prabhudesai2023understanding}.
Explanations and Transparency.




















Schoefer et al.~\cite{schoefer2024explanations} assess how feature-based explanations affect distributive fairness and the mechanisms underlying this effect.
They assess that if explanations highlight the task-relevant features, it impacts users to counter AI recommendations more closely.


Apart from AI systems, research also focuses on understanding users to adapt systems. 

In addition, CFF and frictional AI slow down users' thinking process by adding friction or design interventions.

Domains and tasks show a wide range of applications in educational, business, healthcare, and leisure-related activities. 

exploring that explanations reduce over-reliance without CFFs, noting people's rationale to choose whether or not to engage with AI in a cost-benefit framework.


Salimzadeh et al.~\cite{salimzadeh2024dealing} explore the effect of task complexity and task uncertainty.

Tasks, where human-AI performance is comparable, are more optimal for human-AI-assisted decision-making~\cite{bansal2021does, morrison2023evaluating, vasconcelos2023explanations}. 
If AI is far superior, it is hard to elicit user behavior as they can almost always agree with the models knowing that they have higher odds of getting the correct outcome~\cite{zhang2020effect}. 
Such a setup can work if the objective is to only increase users' trust in the system. 


Subjective trust can promote objective reliance, but such measures can give an overly optimistic image of reliance~\cite{he2023stated}.

The review shows no clear indication that research has established a framework to study human-AI reliance, except few task and user-dependent methods. 

Over-reliance is a known concern; however, research shows limited progress towards unified frameworks to study appropriate reliance.


Hence, enhancing individuals' understanding of self-expertise through accurate mental models can be valuable for forming correct reliance~\cite{cabrera2023improving, he2023knowing, ma2024you}.

However, training and experimentation with real-world experiments at a large scale would be difficult to test, but would extract deeper knowledge.


In addition, AI systems can also highlight the errors earlier, which Nourani et al.~\cite{nourani2021anchoring} explore in limited experiments.

Chen et al.~\cite{chen2023understanding} explore the types of intuition involved in engaging with AI decision-support to explore intuition-driven pathways.

Many times, it becomes difficult to observe model performance due to future events or decisions~\cite{lu2021human}.
AI models should be adaptive to tasks and ML outputs; e.g., using higher confidence when humans and AI are correct and agree with each other, and potentially enable experts to teach models for the other cases~\cite{lu2021human}.

How AI dynamics are displayed to users also affects their performance, for example, higher model confidence was associated with a higher likelihood of a switch~\cite{cao2024designing}.

Without tasks that have comparable performance, we can strip humans or AI away and delegate the task to the other~\cite{bansal2021does}.

Some factors are not controllable by users without task expertise, and in crowd-sourcing~\cite{salimzadeh2024dealing}. 

Explanations of an AI should help people recognize the uncertainty underlying an AI prediction and nudge people to rely on predictions when the model's confidence is calibrated~\cite{wang2021explanations}.

For instance, Wang and Yin~\cite{wang2021explanations} list desirable properties of XAI as 1) understandable, 2) uncertainty aware, and 3) trust calibrated. 
Hence, explanations should be designed in a way that improves people's understanding and skills~\cite{buccinca2025contrastive}.

Tasks can have different levels of uncertainty, which require user expertise, and can vary in reliance on the AI system depending on the level of complexity and uncertainty in the task~\cite{salimzadeh2024dealing}.


For example, design should create just enough friction to switch someone from having their behavior driven by System 1 to System 2~\cite{cox2016design}. 

A positive first impression of the AI results in a higher overall performance than a negative first impression~\cite{vered2023effects}.

It measures users' acceptance of correct AI advice and rejection of incorrect AI advice~\cite{schemmer2023appropriate}.


Nourani et al.~\cite{nourani2021anchoring} also show that model performance can induce \textit{anchoring bias}.


Intervention-generated inequalities (when an intervention favors a group over others) do not help extract realistic behavior~\cite{buccinca2021trust}.


==> x_commented.tex <==
% The rest of the paper is structured as follows: Section~\ref{sec-background} reviews related work and explicitly positions our work in the trust and reliance spectrum. 
% We discuss our rigorous methodology in Section~\ref{sec-method}, highlighting the protocol for collecting and assessing research studies. 
% Section~\ref{sec-analysis} presents our analysis across dimensions, presenting current trends, limitations, and future directions. 
% Section~\ref{sec-discuss} discusses the implications of this work and consensus on the research agenda.
% Finally, we explore limitations and future research directions before concluding this work.
% Overall, summaries of identified dimensions are included in the appendix for a categorical understanding of the work. 



% \textcolor{red}{Particularly, excluding the effects of interventions about AI on user performance, trust, and comprehension from a one-sided perspective of users or the system. But rather on two-way reliance for the correctness of decisions. Also, exclude how imperfections in advice affect user behavior.
% Also, decision-making between AI and humans is a must; explain some of this.
% Most research with LLMs captures users' acceptance of the text or content in general, without any decision-making involved. It could also be excluded.}



% COME HERE
% buccinca2021trust Section 2: Explains cognitive forcing. Dual process theory.
% % nourani2021anchoring Section 5.2: For designers. 
% Types of explanations: 2.1 and 2.2 schoefer2024explanations
% Section 2.1: Good points to follow. de2025cognitive
% Section 5: de2025cognitive
% Some good points in section 2. he2025conversational
% Good points in Section 7: jeon2025empowering
% Some good points on personalization in section 2. swaroop2025personalising
% Very good deskilling in Section 2.2. buccinca2025contrastive

% Some good in Section 7.  ma2024you

% thinking fast and slow. Hence, research informs patterns that enhance human reliance or have not been found useful. % Few studies focus on it. What recent work was introduced?
% We identify methods for delaying thinking.
% While large-scale experiments with a knowledgeable population are hard and expensive. Hence, actual tasks with prolonged deployments can be an effective strategy.


% Read section 5: again and again: cabitza2024never


% More focus on behavioral science and psychology theories can elicit users' behavior.
% While various studies now have defined appropriate objective reliance, the HCI community should make collective efforts to define standardized frameworks for measuring reliance, and reduce focus on subjective trust in reliance studies. For example, linking to Schemmer et al or Cabitza et al. works.

% Future work also needs to look at behavioral theories in interaction design. Multi-step decisions, Multi-option decisions, Hedge and Verify.
% UX can be enhanced to reduce the effect of friction. But limited work has focused on that.
% What we find can be done.
% Threats to validity: Controlled studies. More factors in actual decision-making.
% Run long studies, real-world interactions.



% \textcolor{red}{why our work is important. what existing work covers, what they lack; XAI, Lai et. al, ACM trust.}
% \textcolor{red}{what contribution does this work make}




% \textcolor{red}{overview and differentiating AI reliance from other forms}
% \textcolor{red}{related work on enhancing ai reliance}
% \textcolor{red}{contrasting limited work and there-lack-of human ai reliance in hcai}



% \textcolor{red}{AI Systems: XAI, ML Model Performance. Tasks}
% \textcolor{red}{Interaction: , Learning. CFF, Friction, Effort.}
% \textcolor{red}{Users: Mental Models, Expertise, Knowledge. Behavior (Motivation), Self-Assessment.}


\subsection{Studying Appropriate Reliance}
\label{sec-4-1}
%We assess the different \textbf{components} used to study appropriate reliance. 
Broadly, studies have focused on \textbf{three main directions} for enhancing appropriate reliance on AI, namely 1) \textbf{AI systems} (e.g., by improving performance, uncertainty, explanations)~\cite{bansal2021does, zhang2020effect, buccinca2020proxy, wang2021explanations, yin2019understanding, salimzadeh2024dealing, prabhudesai2023understanding}, 2) \textbf{user factors} (e.g., focusing on expertise, cognitive biases, traits)~\cite{chiang2022exploring, nourani2021anchoring, rastogi2022deciding, vered2023effects, swaroop2024accuracy, swaroop2025personalising, vasconcelos2023explanations, he2023knowing, ma2024you}, and 3) \textbf{interaction factors} (e.g., focusing on enhancing engagement, or changing the behavior of the user towards the tasks)~\cite{buccinca2021trust, cabitza2023ai, de2025cognitive, cabitza2025oracular}. Figure~\ref{fig-mind-map} illustrates an overall categorization of these three directions that the evaluated AI-reliance literature has focused on, and their sub-categories.


\subsubsection{AI System Factors}
\label{sec-4-1-1}
Around 64\% (36) of the studies specifically focus on \textbf{enhancing the AI system}, for example, by improving its performance or augmenting the explanations regarding its functionality (XAI), to support user reliance.
Approximately 13 (23\%) of the studies use AI performance metrics like model confidence and uncertainty~\cite{prabhudesai2023understanding, cau2023effects, cau2023supporting, ma2024you}, as well as accuracy~\cite{yin2019understanding, zhang2020effect} to understand user behavior.
For example, Zhang et al.~\cite{zhang2020effect} study the impact of \textit{model confidence}, which helps calibrate people's trust in AI models.
Making users aware of system capability~\cite{yin2019understanding, zhang2020effect, ma2024you, he2023stated} and uncertainty~\cite {prabhudesai2023understanding, kim2024m, cao2024designing} is important; this is achieved by, for instance, conveying model accuracy on the dataset.
Communicating about uncertainty in the AI system's capacities can help users gauge the pitfalls of model performance and associated risks. However, it can also give them a \textit{false impression} of high confidence. Specifically, accuracy metrics can impact people's trust and reliance, with users reporting higher \textit{trust} in the model when they can compare \textit{their own} accuracy to that of the \textit{system}~\cite{he2023stated}.

With the majority of the studies using XAI, we find that around 57\% (32) of them focus on \textbf{adapting the XAI} method used.
These studies use (experiment) conditions to test the effect of feature-based~\cite{wang2021explanations, wysocki2023assessing, vered2023effects, he2025conversational}, example-based~\cite{nourani2021anchoring, cao2022understanding, tejeda2022ai, cabitza2024never}, model-based~\cite{grgichlaca2019human, chiang2022exploring, brachman2022reliance, peng2024human}, or general explanations methods~\cite{sangdeh2021manipulating, morrison2023evaluating, salimzadeh2024dealing}.
In addition, studies attempt to adapt explanation methods by changing their medium (text, visual)~\cite{yang2020how, morrison2024impact}, complexity (easy to complex)~\cite{vasconcelos2023explanations}, context (analogies, reasoning styles)~\cite{he2023stated, cau2023effects}, or model confidence~\cite{swaroop2025personalising}. 
For instance, model-based explanations may be used if the model is sensitive to the dataset~\cite{zhang2020effect}, explanations adapted to AI's confidence may be used if the model is focused on prediction~\cite{bansal2021does}, or, if the model is focused on user performance, the explanations may be adapted in terms of \textit{when} they are shown to the user~\cite{swaroop2024accuracy}.

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figs/chi-rev-method-overview_new.pdf}
  % \includegraphics[height=16cm]{figs/chi-rev-method-overview.pdf}
  \caption{Overview of the methods and concepts used for appropriate reliance adopted in the final corpus. Studies adapt AI systems, such as their performance and explanations, to influence users to engage with AI advice. This includes understanding the effects of model performance and XAI methods on users' reliance behavior. Research also explores understanding user cognitive factors and self-assessments measuring users' mental models, biases, personality, expertise, and confidence. In addition, research investigates how adapting AI interaction through various engagement-enhancing methods, such as cognitive forcing or motivating/enabling users to perform better and build appropriate reliance.}
  \Description{Figure 4. The figure shows a mind map of methods. The methods are divided into three main categories. AI systems, User Factors, and Interaction Factors. AI systems are further divided into performance factors and XAI methods, which are listed in more detail, like XAI analogies, visual explanations, counterfactuals, XAI difficulty, pro-hoc, post-hoc, local, and global explanations. Performance factors have model uncertainty and accuracy sub-factors. Interaction factors are divided into interventions and motivating adaptations. Interaction adaptations are cost, benefit, XAI utility, partial XAI, time effect, task difficulty, uncertainty, cognitive forcing, frictional AI, and multi-step decision. Motivating factors include user competence, incentivization, performance feedback, and user training. User factors include cognitive factors and user self-evaluations. Cognitive factors include mental models, intuition, user traits, motivation, and cognitive biases like automation bias and algorithmic aversion. User self-evaluation has domain expertise, self-assessment, confidence, uncertainty, literacy, and illusion of AI performance.}
  \label{fig-mind-map}
\end{figure*}

Approximately two-thirds of the studies (38) use \textit{local model explanations}~\cite{zhang2020effect, vered2023effects, schoefer2024explanations} as compared to (13 studies) \textit{global explanations}~\cite{yin2019understanding, grgichlaca2019human, chiang2022exploring, he2023stated}.
Meanwhile, 22 (non-exclusive) studies use \textit{example-based}~\cite{yang2020how, cao2022understanding, cao2022understanding, schemmer2023towards} explanations, while a few use \textit{counterfactual or contrastive explanations}~\cite{buccinca2025contrastive, lee2023understanding, cabitza2024never}.
Counterfactuals focus on the distinctions between the AI's suggestion and a likely human response while highlighting only the dimensions in which the two choices differ~\cite{buccinca2025contrastive}.
Bu\c{c}inca et al.~\cite{buccinca2025contrastive} study the benefits of contrastive explanations to enhance human skill on the task (i.e., human learning), comparing with unilateral explanations.
To reduce the bias towards one advice or explanation, Cabitza et al.~\cite{cabitza2024never} use \textit{``pro-hoc''} explanations (examples and counterfactuals) as a way to present multiple answers instead of AI advice to reduce inappropriate reliance.

Inappropriate reliance can also occur in the presence of \textbf{imperfect XAI}~\cite{morrison2024impact}, a phenomenon where an explanation reveals evidence that does not necessarily comply with the prediction.
Some studies~\cite{he2023stated, cau2023effects} adapt reasoning (analogies, inductive, deductive) of explanations, which show mixed effects on the reliance. 
Overall, these studies show how AI systems are adapted to users; however, there are various trade-offs with each method, and when complemented with user factors, the AI systems should be carefully evaluated to formulate what information should be explained.


\textbf{The debate whether explanations increase or decrease reliance is ongoing}~\cite{bansal2021does, buccinca2021trust, vasconcelos2023explanations, de2025cognitive}.
Vasconcelos et al.~\cite{vasconcelos2023explanations} discussed that the cost of engaging with explanations  (i.e., user difficulty with XAI) can determine the user's reliance. 
For example, if understanding the explanation is equally or more complex than understanding the AI decision, users might refrain from it.
Schoefer et al.~\cite{schoefer2024explanations} found that if explanations highlight the task-relevant features, it impacts users to engage with AI recommendations more closely.
Over-reliance due to explanations can be calibrated with system confidence and uncertainty communication~\cite{vasconcelos2023explanations}.


\subsubsection{User Factors}
\label{sec-4-1-2}
Users have different biases towards automation and AI systems, which come into play when relying on AI advice.
We find that around 23\% (13) of studies explore various biases, including \textit{automation bias}~\cite{nourani2021anchoring, vered2023effects} and \textit{algorithmic aversion}~\cite{cabitza2023ai, pareek2024effect}.
For instance, users may form a misbelief that they understand how the model works when they do not~\cite{nourani2021anchoring, bansal2021does}.
Users may also develop an aversion to AI, being skeptical of the system due to their negative first impressions~\cite{nourani2021anchoring}, thus under-relying on its advice.
In addition, users might not be motivated enough to engage with AI advice, and thereby accept any system advice that comes their way~\cite{vasconcelos2023explanations}.

Prior studies~\cite{green2019principles} in human-AI decision-making have shown that \textbf{cognitive biases} affect people's interaction with AI advice.
For example, the order of observing accurate and inaccurate predictions affects the user's mental model~\cite{nourani2021anchoring}.
Research aims to understand the users' mental models~\cite{prabhudesai2023understanding, cabrera2023improving, ma2024you} to better predict their behavior, and subsequently design interventions.
An important trait for improving the users' mental models concerning AI is capturing their \textbf{``Need for Cognition''}~\cite{cacioppo1982need}, a stable personality trait that captures one's motivation to engage in effortful mental activities~\cite{buccinca2021trust}.
Exploring mental models, AI can be \textit{delegated} to solve easier problems, and users can be engaged for difficult ones, for instance, to recognize AI errors~\cite{brachman2022reliance,bansal2021does}.

Aside from mental models, other mediators affecting reliance on AI include \textbf{personality} traits~\cite{swaroop2024accuracy, swaroop2025personalising}, \textbf{intuition}~\cite{chen2023understanding}, and
self-perceived \textbf{expertise}, which can all influence decision-making~\cite{nourani2020role, he2023stated}. 
We find that around 18\% (10) of studies model and try to calibrate users' self-evaluation, such as their perceived degree of expertise~\cite{dikmen2022effects}, awareness~\cite{he2023knowing, ma2023should, ma2024you}, confidence~\cite{jeon2025empowering}, literacy~\cite{chiang2022exploring}, and their uncertainty~\cite{prabhudesai2023understanding}.
While self-assessing, users can also create an \textit{illusion of AI performance}~\cite{he2023knowing} that can downgrade their performance as people often consider their judgment as a reflection of reality \textbf{({``naive realism''}~\cite{ross2013naive})} without knowing their limitations, leading to over-reliance on models~\cite{lu2021human}. 
As expertise is an essential criterion to influence biases and reliance on the AI advice~\cite{cao2024designing}, Zhang et al.~\cite{zhang2020effect} try to enhance \textbf{users' expertise} by providing additional information.
Dikmen and Burns~\cite{dikmen2022effects} provide \textbf{domain knowledge}, such as contextual data and statistics, to improve expertise, but having no real incentives or the risk of making wrong decisions affects users' behavior. 

A few studies~\cite{chiang2022exploring, he2023knowing, he2024err} looked at providing XAI \textbf{tutorials} to convey AI performance and enhance users' abilities.
Chiang and Yin~\cite{chiang2022exploring} show that users need to understand and learn ML systems before they can effectively engage with them, allowing users to construct their datasets and tests to improve their mental models.
Tests can identify possible disparities in data, and users can learn about these disparities before experimenting with tasks~\cite{cau2025influence}.
Users also face inherent issues with the complexity of explanations. For example, feature-based explanations (summing up feature effects) to show model confidence are not obvious for people without sufficient AI expertise to understand the underlying models~\cite{zhang2020effect}.
Users may find those explanations to be rather foreign and mentally taxing to consume~\cite{wang2021explanations}.

Users could trust an AI model \textit{inappropriately}, and still achieve a higher accuracy (e.g., blindly trust a model that has a higher accuracy than oneself)~\cite{wang2021explanations}.
Conversely, users can overestimate their confidence in decisions due to inaccurate interpretations~\cite{lu2021human}, or cognitive biases (e.g., Dunning–Kruger effect~\cite{kruger1999unskilled}: people overestimate their abilities), leading to under-reliance on the ML models.
For non-expert users, gaps in domain knowledge can lead to misunderstandings~\cite{dikmen2022effects}, which can subsequently affect the collaboration strategy~\cite{bansal2021does}. 
Hence, understanding user factors is critical to conducting human-AI experiments and designing interventions to better adapt interactions with AI systems.

\subsubsection{Interaction Factors}
\label{sec-4-1-3}
Most of the research on interaction factors focuses on adapting user interaction with the AI system, drawing from human psychology theories~\cite{wason1974dual, kahneman2011thinking, cox2016design} and implementation design.
For example, interaction can be designed to adapt (to) user behavior~\cite{bansal2021does, swaroop2025personalising, de2025cognitive} or system functionality~\cite{buccinca2021trust, buccinca2020proxy}.
We find that 70\% (39) of the examined studies adapt the interaction through intervention methods (10 studies) or motivating factors (29 studies). 
A common method is using cognitive forcing functions (CFFs)~\cite{de2025cognitive, buccinca2021trust, jeon2025empowering}  or frictional AI~\cite{cabitza2023ai, cabitza2024never, cabitza2025oracular} to \textbf{add delays} to user engagement with AI.
People employ dual process theory~\cite{kahneman2011thinking, wason1974dual}, quick (system 1) or analytical (system 2) thinking when interacting with tasks.
Bu\c{c}inca et al.~\cite{buccinca2021trust} use CFFs to increase people's \textbf{cognitive motivation} for engaging analytically with AI explanations.
CFFs are used in frictional design~\cite{naiseh2021nudging, cox2016design}, which add delays or slow downs to force users to use (system 2) \textbf{analytical thinking}~\cite{cabitza2023ai, jeon2025empowering, cabitza2025oracular}. 
In similar lines, de Jong et al.~\cite{de2025cognitive} employ \textbf{partial explanations} as a way to increase user engagement with XAI.
Ma et al.~\cite{ma2025towards} introduce \textbf{human-AI deliberation} as a way to discuss conflicting opinions between AI and humans to create evidence-based decision updates for AI or users.
Combining with \textbf{slowdown interventions}, studies explore adapting the decision-making approaches, such as \textit{multi-step decisions}~\cite{schemmer2023towards, tejeda2022ai}, evoking or overcoming users' biases towards or against the AI advice.

Studies also engage users to enhance their competence~\cite{chiang2022exploring, brachman2022reliance, cao2022understanding}, such as through \textbf{training}, or by providing performance feedback~\cite{yin2019understanding, grgichlaca2019human}.
However, due to factors such as task expertise and users' relevance with the tasks, \textit{training methods} have not contributed significantly towards reliance~\cite{salimzadeh2024dealing}.
Some (9) studies provide performance feedback to users to reassure their decisions; however, others reason that this is not a viable representation of the real world, as decision feedback is not instant but comes in the future.
In some cases, the feedback is provided during the training tasks, and not during the actual experiment.
Another commonly explored method (29 studies) is to improve engagement by enhancing the users' incentives, although with a meager value.
For instance, many studies~\cite{yin2019understanding, cau2023supporting, salimzadeh2024dealing, swaroop2024accuracy, he2025conversational} explore \textbf{extrinsic incentives}, such as monetary rewards, to improve performance; however the use of such incentives rarely achieves the intended outcomes~\cite{grgichlaca2019human, wysocki2023assessing}. 
Hence, incentives, at the current rate, have not been very effective in enhancing users' reliance on AI advice.

Sandbox environments~\cite{chiang2022exploring, he2024err} are used to evaluate users' engagement with model predictions, where \textit{interactivity} or \textit{agency} can enhance people's understanding and perceived usefulness of the system.
Studies also add time pressure~\cite{cao2023time, swaroop2024accuracy, swaroop2025personalising, rastogi2022deciding} to understand engagement for reliance under constraints.
Interaction methods are adapted to add task constraints such as complexity or uncertainty of tasks~\cite{salimzadeh2024dealing}. 
Engagement can also make people evaluate a model's predictions~\cite{sangdeh2021manipulating}; however, without the model's information, people's reliance depends on alignment with the model's prediction~\cite{lu2021human}.
Overall, adapting interaction to users' performance and cognition, and AI's performance and confidence has been found useful~\cite{buccinca2021trust, cabitza2023ai, cabitza2025oracular, de2025cognitive}, but engaging users to elicit realistic behavior is still a challenging task.

\textbf{Key insights}: The literature has focused on three main directions to improve user reliance on AI. The first one concerns \textbf{AI Systems}, where studies have explored various XAI methods, XAI delivery mediums, and XAI complexity levels, without a conclusive, however, consensus emerging on whether explanations increase or decrease reliance. Secondly, the literature has explored \textbf{user factors}, examining how human biases and other traits (e.g., personality, intuition, and self-perceptions) affect user reliance on AI. Notably, users' ``need for cognition'' can be used to predict whether users will meaningfully engage with AI.
Third, the literature has looked into \textbf{interaction Factors}, with a notable finding that cognitive forcing and frictional designs show a positive impact towards users' reliance on AI; however, extrinsic incentives, such as monetary rewards, do not appear to contribute towards appropriate reliance.

